Type-Constrained Code Generation with Language Models

Large language models (LLMs) have achieved notable success in code generation. However, they still frequently produce uncompilable output because their next-token inference procedure does not model formal aspects of code. Although constrained decoding is a promising approach to alleviate this issue, it has only been applied to handle either domain-specific languages or syntactic features of general-purpose programming languages. However, LLMs frequently generate code with typing errors, which are beyond the domain of syntax and generally hard to adequately constrain. To address this challenge, we introduce a type-constrained decoding approach that leverages type systems to guide code generation. For this purpose, we develop novel prefix automata and a search over inhabitable types, forming a sound approach to enforce well-typedness on LLM-generated code. We formalize our approach on a foundational simply-typed language and extend it to TypeScript to demonstrate practicality. Our evaluation on the HumanEval and MBPP datasets shows that our approach reduces compilation errors by more than half and significantly increases functional correctness in code synthesis, translation, and repair tasks across LLMs of various sizes and model families, including state-of-the-art open-weight models with more than 30B parameters. The results demonstrate the generality and effectiveness of our approach in constraining LLM code generation with formal rules of type systems.

==> Makefile <==
# Makefile, allowing to
# - compile
# - test
# - clean
# - run in docker
# For details, see targets defined below
#
# USAGE, for example: make pdf

#####################
# REQUIRED PACKAGES #
#####################

# For instructions on how to set up your system to run all commands here, follow
# https://hub.docker.com/repository/docker/ethsrilab/latex-plus

##############
# PARAMETERS #
##############

# main
OUTPUTDIR := lqa-output
NAME := main
SUBMISSION := submission
SUPPLEMENT := submission_supplement

# special
OVERFULL := $(NAME)_overfull
GRAY := $(NAME)_gray

# submission
SUBMISSIONDIR := final_submission
ZIP := submission.zip

# log
LATEXMKDIR := $(OUTPUTDIR)/latexmk
LOG := $(LATEXMKDIR)/$(NAME).log
SHORTLOG := $(OUTPUTDIR)/$(NAME)-short.log
OVERFULLOUTPUTDIR := $(OUTPUTDIR)/overfull

LOGFILES := *.aux *.bbl *.log *.bcf  *.blg *.lot *.toc *.swp *.gz *.out *.ttt *.fls *.fdb_latexmk

# scripts

SCRIPTDIR := lqa/scripts

#############
# COMPILING #
#############

LATEX         := ./lqa/latex.sh $(NAME).tex $(LATEXMKDIR)
LATEXOVERFULL := ./lqa/latex.sh $(OVERFULL).tex $(OVERFULLOUTPUTDIR)

##########
# OTHERS #
##########

# latex code to enable marking overfull areas
OVERFULLFILECONTENT := \def\isoverfull{1} \input{$(NAME).tex}

########
# PDFS #
########

.DEFAULT_GOAL := pdf

.PHONY: pdf
pdf:
	@echo "\n> COMPILING pdf..."
	$(LATEX)
	@cp $(LATEXMKDIR)/$(NAME).pdf $(OUTPUTDIR)
	@cp $(LATEXMKDIR)/$(NAME).pdf .
	@cp $(LOG) $(OUTPUTDIR)

.PHONY: overfull
overfull:
	@echo "\n> COMPILING OVERFULL pdf..."
	echo "$(OVERFULLFILECONTENT)" > $(OVERFULL).tex
	$(LATEXOVERFULL)
	@cp $(OVERFULLOUTPUTDIR)/$(OVERFULL).pdf $(OUTPUTDIR)
	rm $(OVERFULL).tex # cleanup

# make split: builds the whole paper and splits it into submission and supplementary material
.PHONY: split
split: pdf
	python $(SCRIPTDIR)/pages.py --action split

.PHONY: gray
gray: pdf
	@echo "\n> Producing GRAYSCALE version to $(OUTPUTDIR)/$(GRAY).pdf..."
	gs -sOutputFile=$(OUTPUTDIR)/$(GRAY).pdf -sDEVICE=pdfwrite -sColorConversionStrategy=Gray -dProcessColorModel=/DeviceGray -dCompatibilityLevel=1.4 -qQUIET -dNOPAUSE -dBATCH $(OUTPUTDIR)/$(NAME).pdf

# produce better log files
.PHONY: log
log: pdf
	pplatex -i $(LOG) > $(SHORTLOG)

.PHONY: printlog
printlog: log
	cat $(SHORTLOG)


###############
# CONVENIENCE #
###############

.PHONY: check
check: pdf log
	python $(SCRIPTDIR)/checks.py

.PHONY: all
all: pdf split gray check log overfull

#########
# CLEAN #
#########

.PHONY: clean
clean:
	@echo "\n> CLEANING temporary files..."
	cd $(OUTPUTDIR) && rm -f $(LOGFILES) || true
	rm -f $(LOGFILES) || true
	rm -r -f $(LATEXMKDIR) $(OVERFULLOUTPUTDIR) || true
	rm -r -f $(OUTPUTDIR)/script-logs/*.log* || true

# make cleanall: remove all produced files
.PHONY: cleanall
cleanall: clean
	@echo "\n> CLEANING PDFs..."
	rm -f *.pdf || true
	rm -f $(OUTPUTDIR)/*.pdf || true
	rm -r -f $(SUBMISSIONDIR) || true

##############
# SUBMISSION #
##############

.PHONY: abstract
abstract:
	python $(SCRIPTDIR)/abstract.py

# prepare a submission: produce PDFs and ZIP
.PHONY: submission
submission: split check
	@echo "\n> PREPARING submission in directory $(OUTPUTDIR)..."
	rm -r -f $(SUBMISSIONDIR)
	mkdir $(SUBMISSIONDIR)
	cp $(OUTPUTDIR)/$(SUBMISSION).pdf $(SUBMISSIONDIR)
	cp $(OUTPUTDIR)/$(SUPPLEMENT).pdf $(SUBMISSIONDIR)
	cp $(LATEXMKDIR)/$(NAME).bbl $(SUBMISSIONDIR)

# zip the whole directory and place the result in /submission
.PHONY: zip
zip: submission
	@echo "\n> ZIPPING directory..."
	@rm -f $(SUBMISSIONDIR)/$(ZIP)
	zip --quiet -r $(SUBMISSIONDIR)/$(ZIP) . -x /.git* /$(OUTPUTDIR)* /$(SUBMISSIONDIR)/*.zip

##########
# DOCKER #
##########

DOCKER := ./lqa/docker.sh


PAPERDIR := $$(pwd)
IMAGE := ethsrilab/latex-plus:version-4.0
CONTAINER := latex-plus-container
RUN := $(DOCKER) run \
		-it \
		--name $(CONTAINER) \
		--workdir="/paper" \
		-v $(PAPERDIR):/paper \
		$(IMAGE)

# launch a docker container using the image, which will provide a shell in the container
.PHONY: docker-run
docker-run: clean-container
	$(RUN)

# check for updates and remove the created docker container
.PHONY: clean-container
clean-container:
	$(DOCKER) pull $(IMAGE)
	$(DOCKER) rm /$(CONTAINER) 2>/dev/null || true

# all above commands, run in docker
.PHONY: docker-all
docker-all: clean-container
	$(RUN) make all

.PHONY: docker-pdf
docker-pdf: clean-container
	$(RUN) make pdf

.PHONY: docker-overfull
docker-overfull: clean-container
	$(RUN) make overfull

.PHONY: docker-split
docker-split: clean-container
	$(RUN) make split

.PHONY: docker-gray
docker-gray: clean-container
	$(RUN) make gray

.PHONY: docker-check
docker-check: clean-container
	$(RUN) make check

.PHONY: docker-zip
docker-zip: clean-container
	$(RUN) make zip
	
.PHONY: docker-abstract
docker-abstract: clean-container
	$(RUN) make abstract



==> figures/grammar/grammar.tex <==
\begin{figure}[tp]
  \small
  \centering
    %\hfill
    %  \hspace{10ex}

  \begin{subfigure}[t]{0.48\textwidth}
  \centering
  \begin{tabular}{@{}p{\textwidth}@{}}
    \begin{grammar}
    <l> ::= "\textbackslash d+" | "\"\textbackslash w*\"" | "true" | "false"

    <x> ::= "\textbackslash w+"

    <p> ::= <x> : T

    <T> ::= "number" | "string" | "boolean" | "(" <\textoverline p> ") =>" <T>

    <e> ::=  <l> \ | <x> | \ "(" <\textoverline p> ") =>" <e> \ | \ "(" <e> ")" \ | <e> $\circ$ <e> | <e> "(" <\textoverline e> ")" | <e> "." <n> 
   \end{grammar}
  \end{tabular}
  \end{subfigure}
    \hspace{3ex}
\begin{subfigure}[t]{0.35\textwidth}
  \centering
      \begin{tabular}{@{}p{\textwidth}@{}}
    \begin{grammar}
    <s> ::=  "{" <\textoverline s> "}"
    \alty "let" <x> ":" <T> ";" 
    \alty <e>  ";"
    \alty "if (" <e> ")" s " else " s
    \alty "function" <x> "(" <\textoverline p> ") :" <T> "{" <\textoverline s> "}"
    \alty "return" <e> ";"

    <M> ::= <\textoverline s>
   \end{grammar}
  \end{tabular}
  \end{subfigure}
  \vspace{-5mm}
  \caption{The grammar for identifiers $x$, literals $l$, expressions $e$ and types $T$ (left), and statements $s$ and the complete program $M$ (right) in \subts{} follows standard definitions. $x$ and $l$ are based on regular expressions.}
  \label{fig:subset-l}
\end{figure}


==> lqa/scripts/tests/abstract/header.tex <==
%%%%%%%%%%%%%%%%%
% ABBREVIATIONS %
%%%%%%%%%%%%%%%%%


\newcommand{\eg}{e.g., }
\newcommand{\tool}[0]{\emph{Sometool}\xspace}


==> lqa/scripts/tests/header/cmd.tex <==
abc

\newcommand{\cmd}[0]{cmd}


==> lqa/scripts/tests/header/package.tex <==
abc

\usepackage{abc}


==> lqa/scripts/tests/helpers/main.tex <==
x1
% x2
x3 % x4
x5 \% x6
x7\begin{comment}
x8
\end{comment}x9
x10


==> lqa/scripts/tests/hyphenation/check.tex <==
These occurrences should be fine:

We compute it in constant-time successfully.
We achieve state-of-the-art results.
May hyphenated words may occur at sentence-end?
Hyphenated words may occur at sentence-end.
Hyphenated words may occur at sentence-end!
single-occurrence
occurrence-one occurrence-two
multiple real-worlds

These occurrences should be reported:

We should not write constant time here.
single occurrence
We should not write state-of-the art.


==> lqa/scripts/tests/hyphenation/parse.tex <==
We compute it in constant-time successfully.

We achieve state-of-the-art results.

May hyphenated words may occur at sentence-end?

Hyphenated words may occur at sentence-end.

Hyphenated words may occur at sentence-end!

single-occurrence

occurrence-one occurrence-two

multiple real-worlds

should ignore this: $a-b$

==> lqa/scripts/tests/merge_msgs/merge_msgs.tex <==
Hello world

<<<<<<< HEAD
this is some content to mess with
content to append

=======
totally different content to merge later
>>>>>>> 0489das287d4639d049dddas
that's it


==> lqa/scripts/tests/parse_latex/parser-body.tex <==
\section{My section}

Hello world! This is just an example text that spans multiple lines,
which we can hopefully parse correctly. Even the \emph{third} line should
work if the developers did a good job.

Also a second paragraph goes here. We present \systemname, the first tool
to automatically perform great tasks.

\paragraph{First step} Read this fancy paragraph that even contains
math $x < 3$ in it! There is some continuation of this text, which
should be merged together with part of the text that comes before
the inlined math.

The following formula
\[
    e = mc^2    
\]
is inlined into a sentence.

\begin{figure}
    \centering
    This is a figure content
    \caption{This is a caption}\label{fig:sample-label}
\end{figure}

\begin{enumerate}
    \item First item containing \emph{emphasis} in it % and a comment
          and continues here
    \item Second item
\end{enumerate}

==> lqa/scripts/tests/parse_latex/parser-header.tex <==
\usepackage{xcolor} % for definecolor
\usepackage{amsthm, amsmath}

\newcommand{\systemname}[0]{MySystem}
\newcommand{\eg}[1]{\emph{e.g.,~}}


==> lqa/scripts/tests/references/eqref.tex <==
abc \eqref{def}


==> lqa/scripts/tests/references/ref.tex <==
abc \ref{def}


==> lqa/scripts/tests/unreferenced_floats/floats.tex <==
\section{My section}\label{sec:section}
Hello! We are now referencing \cref{fig:example} and also \cref{tab:example}, but nothing else.

\lstinputlisting[caption={Example code.},label=lst:example]{inexistent.java}

\begin{figure}
    Test
    \caption{Some caption}\label{fig:example}
\end{figure}

\begin{table}
    Test
    \caption{Some caption}
    \label{tab:example}
\end{table}

\begin{figure}
    Test
    \caption{Some caption}
    \label{fig:example_missing}
\end{figure}

\begin{table}
    Test
    \caption{Some caption}\label{tab:example_missing}
\end{table}
